Jet energy measurement and its systematic uncertainty in proton-proton collisions at $\sqrt{s}=7$ TeV with the ATLAS detector

The jet energy scale (JES) and its systematic uncertainty are determined for jets measured with the ATLAS detector using proton-proton collision data with a centre-of-mass energy of $\sqrt{s}=7$ TeV corresponding to an integrated luminosity of 4.7 fb$^{-1}$. Jets are reconstructed from energy deposits forming topological clusters of calorimeter cells using the anti-k$_t$ algorithm with distance parameters $R=0.4$ or $R=0.6$, and are calibrated using MC simulations. A residual JES correction is applied to account for differences between data and MC simulations. This correction and its systematic uncertainty are estimated using a combination of in situ techniques exploiting the transverse momentum balance between a jet and a reference object such as a photon or a Z boson, for $20 < p_T < 1000$ GeV and pseudorapidities $|\eta|<4.5$. The effect of multiple proton-proton interactions is corrected for, and an uncertainty is evaluatedusing in situ techniques. The smallest JES uncertainty of less than $1 %$ is found in the central calorimeter region($|\eta|<1.2$) for jets with $55< p_T< 500$ GeV. For central jets at lower $p_T$, the uncertainty is about $3 %$. A consistent JES estimate is found using measurements of the calorimeter response of single hadrons in proton-proton collisionsand test-beam data, which also provide the estimate for $p_{T,jet} > 1$ TeV. The calibration of forward jets is derived from dijet $p_T$ balance measurements. The resulting uncertainty reaches its largest value of $6%$ for low-$p_T$ jets at $|\eta|=4.5$. Additional JES uncertainties due to specific event topologies, such as close-by jets or selections of event samples with an enhanced content of jets originating from light quarks or gluons, are also discussed. The magnitude of these uncertainties depends on the event sample used in a given physics analysis, but typically amounts to $0.5%$ to $3%$.

==> categoryReduction.tex <==
\subsection{Alternative reduced configurations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
A global reduction of nuisance parameters, irrespective of the uncertainty source, 
is performed in order to reduce the number of these parameters required to represent the full correlation matrix,
see \secRef{sec:simplifiednuisanceParameters}.  
However, it is also useful to keep track of the physical meaning of the uncertainty components,
e.g. for a proper combination of measurements from different experiments.
In \secRef{sec:insitutechniquesuncertainties} each \JES{} systematic uncertainty component
is assigned to a representative category, as given in Table \ref{tab:nuissanceparameters}.
%
%

The same reduction technique discussed in \secRef{sec:simplifiednuisanceParameters} is applied independently to each set of uncertainty components within each individual category.
The resulting reduced set of uncertainty components for the nominal configuration are shown in \figRef{fig:CategoryReduction}. This category reduction approach generally results in a larger 
number of nuisance parameters than the global reduction. This is because two components 
from different categories with very similar shapes can be globally combined without significant loss of information for the correlations. 
%
However, when the reduction is performed in categories, components may require a nuisance parameter not lose 
significant precision for the description of the global correlation.
%

This technique is applied to each of the correlation scenarios. Category reduction configurations 
are derived for the set of all parameters, the stronger correlation scenario, and the weaker correlation scenario.  
In each case, correlation matrices are compared to ensure that the reduction preserved correlation information 
to within a few percent.  Table \ref{table:AllConfigurations} lists the various configurations evaluated,
%
together with the accuracy achieved with the reduction procedure.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
\begin{table*}
\begin{centre}
\begin{tabular}{|l|c|c|c|}
  \hline
  Configuration type & Reduction & $N_{\rm params}$ & Reduction precision (\%) 
  \\\hline
  All parameters & none & $54$ & $100$
  \\\hline
  All parameters & global & $6$ & $97$ 
  \\\hline
  All parameters & category & $11$ & $95$
  \\\hline
  Stronger correlations & none & $45$ & $100$
  \\\hline
  Stronger correlations & global & $6$ & $97$
  \\\hline
  Stronger correlations & category & $12$ & $96$
  \\\hline
  Weaker correlations & none & $56$ & $100$
  \\\hline
  Weaker correlations & global & $6$ & $97$
  \\\hline
  Weaker correlations & category & $12$ & $95$
  \\\hline
  \end{tabular}
  \caption[\JES{} configuration summary]{A summary of the various explored \JES{} configurations. The precision of the reduction is defined by the largest deviation in correlations between the original full set of parameters and the reduced version. The full \pT{} phase space is considered in this determination.
%
%
The values quoted are for jets in the region $|\etajet|<1.2$ 
for \antikt{} with $R=0.4$ calibrated with \EMJES{} scheme. The number of nuisance parameters quoted refers only to the parameters entering the reduction procedure, which are relevant to the \insitu{} techniques.}
  \label{table:AllConfigurations}
\end{centre}
\end{table*}


==> correlationScenarios.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[htp!]
  \centering
  \subfloat[Nominal correlation]    {\includegraphics[width=0.49\textwidth]{figures/AllNuisanceParameters_CorrelationMatrix}\label{fig:CorrelationMatricesFull}}
%
%
  \subfloat[Difference between weaker and stronger correlation]{\includegraphics[width=0.49\textwidth]{figures/Difference_WeakerMinusStronger_CorrelationMatrix.pdf}\label{fig:CorrelationMatricesDiff}}
  \caption[]{
    \JES{} correlation matrix \subref{fig:CorrelationMatricesFull} and the difference between the correlation matrices of the interpretations resulting in stronger and weaker 
    correlations \subref{fig:CorrelationMatricesDiff}
    for \antikt{} jets with $R=0.4$ calibrated using the \EMJES{} calibration scheme in the central calorimeter region ($\etajet=0.5$). 
    \label{fig:CorrelationMatrices}
  }
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Jet energy scale correlation scenarios}

The \JES{} uncertainty and its correlations discussed so far can play a crucial role in physics analyses.  
In order to quantify these correlations, knowledge of the interdependence of the
systematic uncertainty sources is needed. The limitations in this knowledge lead to uncertainties on the correlations. 

The variation of the systematic uncertainty sources as a function of \pt{} and \etajet{} can be described as a nuisance parameter, as explained before.
The total set of correlations can be expressed in the form of a correlation matrix
calculated from the full set of nuisance parameters as presented in \secRef{sec:combinationresults}.
The correlation matrix, derived assuming that the nuisance parameters are
independent from each other, is shown in \figRef{fig:CorrelationMatrices} \subref{fig:CorrelationMatricesFull}. 
%
%

%
The nuisance parameters are affected by the strength of the correlations between uncertainty components, which can be difficult to estimate. The investigation of alternative correlation 
scenarios for the components thus allows to determine the uncertainty on the global correlations shown in \figRef{fig:CorrelationMatrices} \subref{fig:CorrelationMatricesFull}.

%
%
Two additional configurations are specifically designed to weaken and to strengthen the global correlations. They cover the space of reasonable \JES{} component dependencies.
In a given physics analysis these scenarios can be used to examine how the final results are affected by variations of the correlation strengths. This allows propagation of the uncertainties on the correlations.
%
The difference between the weaker and stronger correlation matrices is shown in Figure \figRef{fig:CorrelationMatrices}\subref{fig:CorrelationMatricesDiff}.
%




==> singlehadronresponse.tex <==
The \JES{} correction and uncertainty  derived from \insitu{} techniques exploiting the \pt{} balance between
a jet and a reference object can be compared to the method where the jet energy scale is estimated
from single hadron response measurements, as described in Ref.\cite{jespaper2010}.
In this method, jets are treated as a superposition of energy deposits of single particles.
For each calorimeter energy deposition within the jet cone, 
the type of the particle inside the jet is determined,
and the expected mean shift and the systematic uncertainty of the calorimeter response 
between data and MC simulation is evaluated. 
The corresponding uncertainty is derived from \insitu{} measurements or systematic MC variations.
This deconvolution method is described in Ref. \cite{jespaper2010,eppaper2010} and
is used for the derivation of the \JES{} uncertainty for the \ATLAS{} $2010$ data analysis.

Measurements of the calorimeter response to pions in the combined test-beam \cite{CTB04pion}
are used for pions with momenta between $20$ and $350$ \GeV{}\footnote{The MC simulation was updated from the version used
for the combined test-beam studies to the version used for the collision data simulation.}. 
Single isolated hadrons with momenta up to $20$ \GeV{} are selected in a minimum bias sample 
produced in \pp{} collisions at $\sqrt{s} = 7$~\TeV{} taken in $2011$
and the calorimeter energy ($E$) in a narrow cone around an isolated track is compared
to the track momentum ($p$) (see Refs. \cite{eppaper2010,TauEnergyUncertainty2012} for more details).
Effects from the  noise thresholds and from the calorimeter acceptance are 
estimated by comparing the energy measured in calorimeter cells to the one measured in \topos.
In addition, the uncertainty on the absolute electromagnetic energy scale is considered
and the response uncertainty of protons, anti-protons and neutral hadrons 
is evaluated using different hadronic shower models, again as described 
in Refs. \cite{eppaper2010,TauEnergyUncertainty2012}. 
For hadrons with $p > 400$ \GeV{}, for which no measurements are available in the combined test-beam, 
the uncertainty is conservatively estimated as $10 \%$ to account for possible calorimeter non-linearities 
or longitudinal leakage. 

The mean $E/p$ is well described by the MC simulation for $p>6$ \GeV.
However, for lower momenta ($1 \lesssim  p < 6$ \GeV) the data are shifted down with respect 
to the MC simulation by about $4 \%$.
This is in contrast to the $2010$ measurement, where an agreement within $3 \%$ is found \cite{eppaper2010}. 
The worse data-to-MC agreement is due to the new corrections in the absolute electromagnetic
energy scale obtained \insitu{} using the $Z$ boson mass constraint reconstructed from $Z \to e^+ e^-$,
the increased \topo{} thresholds, and the use of a new \geant{} version.

\FigRef{fig:EOverP}\subref{fig:ep_response} shows the estimated calorimeter jet response ratio 
between data and MC simulation as estimated from the single hadron response
measurements as a function of the jet transverse momentum. 
A lower calorimeter response to jets 
in data than in the Monte Carlo is observed (black circles),
consistent with that obtained using \insitu{} techniques. 
The uncertainty on this ratio is about $4 \%$ at very low and very high \pt. 
It decreases to about $2 \%$ between $100 \le \pt < 600$ \GeV. 
The individual uncertainty components are also shown. The dominant uncertainties
at low \pt{} are those from noise threshold effects, which can be different for single isolated
hadrons and hadrons inside jets. At high \pt{} the response
differences between data and MC simulation as measured in the \ATLAS{} combined
test-beam and the uncertainty for hadrons with $p>400$ \GeV{} are largest.
The uncertainty on the global electromagnetic energy scale and the response
uncertainty for neutral hadrons contribute about $1 \%$.

\FigRef{fig:EOverP}\subref{fig:ep_jes} compares the \JES{} uncertainty as obtained from single hadron
response measurements to the one obtained from the \insitu{} method based on 
the \pt{} balance between a jet and a well-measured reference object.
For both methods the mean jet calorimeter response in data is observed to be shifted down 
by about $2\%$ with respect to the one in the MC simulated events. 
However, the \pt{} balance methods give a considerably smaller uncertainty.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!ht]
  \centering
\subfloat[]{\includegraphics[width=0.49\textwidth]{figures/jesepAll} \label{fig:ep_response}}
\subfloat[]{\includegraphics[width=0.49\textwidth]{figures/epcomparison} \label{fig:ep_jes}}
 \caption[]{Relative calorimeter jet response ratio between data and Monte Carlo simulation,
as estimated from the single hadron response measurements as a function of the jet transverse momentum, is shown in \subref{fig:ep_response}. 
The total systematic uncertainty together with the uncertainty from the individual components
is shown as a lighter band.
The black circles denote the expected mean shift of the calorimeter response to jets in
data over the one of Monte Carlo simulation.  In \subref{fig:ep_jes},  the uncertainty from the single hadron response measurements is shown as a lighter (yellow) band, while
the \JES{} uncertainty, as derived from the \insitu{} methods based on \pt{} balance, is shown as a dark (gray) band. 
The closed markers denote the expected shift of the calorimeter response to jets in data over the one 
in Monte Carlo simulation, and
the line shows the \JES{} correction derived from the \pt{} balance \insitu{} methods.
\label{fig:EOverP}
}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> zjet_Zjetresults.tex <==
\FigRef{fig:ResultsZjetJES} shows the \datatomc{} ratio of the mean \pt{} balance for jets 
calibrated with the \EMJES{} and the \LCWJES{} schemes, with statistical and systematic uncertainties. 
For $R=0.4$ jets and $\pt^{\text{ref}}>25\GeV$, this ratio is shifted by at most $-4\%$ from unity, 
and typically by $-2\%$ over most of the \Zboson{} boson \pt{} range. 
The total uncertainties are typically between $1\%$ and $2\%$ for $25 <\pt^{\text{ref}}<260\GeV$, 
and increase up to $10\%$ for low transverse momenta. 

%





